Inductive Learning of Answer Set Programs from Noisy Examples

In recent years, non-monotonic Inductive Logic Programming has received growing interest. Specifically, several new learning frameworks and algorithms have been introduced for learning under the answer set semantics, allowing the learning of common-sense knowledge involving defaults and exceptions, which are essential aspects of human reasoning. In this paper, we present a noise-tolerant generalisation of the learning from answer sets framework. We evaluate our ILASP3 system, both on synthetic and on real datasets, represented in the new framework. In particular, we show that on many of the datasets ILASP3 achieves a higher accuracy than other ILP systems that have previously been applied to the datasets, including a recently proposed differentiable learning framework.

==> intro_old.tex <==
Over the last two decades, there has been a growing interest in Inductive Logic Programming (ILP)~\cite{Muggleton1991}, and area of supervised learning where the goal is to learn {\em hypotheses} that {\em cover} a set of labelled examples, relative to a given background knowledge. Different ILP frameworks have been proposed in the literature with specific notions of coverage. Traditional ILP has focused on learning definite logic programs required to {\em entail} all positive examples and none of the negative examples. But more recently, ILP has been extended to the field of non-monotonic learning, where hypothesis can be expressed as normal logic programs (e.g.,~\cite{ray2009nonmonotonic}, ~\cite{raspal}, ~\cite{Corapi2010}) or as answer set programs (\cite{Gelfond1988}). The underlying intention is the development of algorithms able to perform automated acquisition of a variety of declarative knowledge, as for instance learning Event Calculus non-monotonic common-sense theories from event sequences as labelled examples (\cite{ILED}, \cite{ICLP15, ICLP16}), or learning theories about scheduling or agents' preferences from labelled examples of past decisions or choices. The non-monotonicity property of these approaches makes them also suitable for learning revisions and adaptations of existing knowledge in response to new evidence or exceptions (e.g., \cite{raspal_thesis}, \cite{Corapi2011} and \cite{ICSE2013}). 

Main advantage of these ILP approaches versus other types of (statistical) machine learning is their ability of learning hypotheses that can be expressed into plain English, so  facilitating close interactions between humans and machine by allowing humans to derive explicit knowledge from machines and machines to learn from humans and other data sources. In particular, recent results in inductive learning of answer set programs, referred as ILASP frameworks (e.g., \cite{ICLP15}, \cite{ICLP16}) have demonstrated the high-level cognitive ability of these systems to support automated acquisition of complex knowledge structures. ILASP has shown to provide several advantages when compared to traditional ILP systems. Firstly, as ASP is highly declarative, procedural constraints do not need to be taken into account when learning structured knowledge. This is instead required by traditional ILP systems where goal directed SLDNF procedure of Prolog must be taken into account specifically when learning knowledge with negation in order to insure that the learned knowledge is expressed as stratified logic programs. No such considerations need to be taken into account when learning ASP programs. A second, more fundamental advantage of the ILASP frameworks is the complex structure of the knowledge that they can learn. This can be expressed using extra types of rules that are not available in traditional ILP as not representable in Prolog, such as choice rules and weak constraints. Learning choice rules allows the learning of non-deterministic concepts. For instance, the concept that a coin may non-deterministically land on either heads or tails, but never both can be learned as a choice rule. Learning weak constraints enables the learning of preference models, as demonstrated in \cite{ICLP15} and \cite{ICLP16}. The increased generality of the learning capability of ILASP frameworks versus traditional ILP  has been formalised and proved in \cite{AIJ17}, with respect to a new notion of coverage of labelled examples. The answer set semantics underpinning the ILASP frameworks allows for acquired knowledge, expressed as answer set programs, to have none, one or even many models (or answer sets~\cite{}). So, coverage can be thought of as entailment of all positive examples from at least one answer set of the learned knowledge with respect to a given background knowledge (i.e. {\em brave induction}), or from all answer sets of the learned knowledge with respect to a given background knowledge (i.e. {\em cautious induction})~\cite{Sakama2009}. In \cite{JELIAILASP}, we have shown that none of these two notions of coverage are sufficient if taken individually.  when learning complex knowledge structures expressed as answer set programs, as there are some ASP programs that cannot be learned by either brave or cautious induction alone. The new notion of coverage of ILASP frameworks unifies brave and cautious inductions by requiring positive examples to be covered bravely and negative examples to be covered cautiously by a learned hypothesis together with a given background knowledge. 

Despite the increase of generality in the notion of coverage, which allows for the learning of more complex knowledge, the underling assumption of existing ILASP frameworks is that of {\em perfect} coverage, meaning that no labelled example must be left uncovered by the learned knowledge.  In practice, examples are unlikely to be perfectly labeled. In real datasets, there is likely to be noise. A more realistic approach in automated knowledge acquisition is therefore the learning of hypotheses that cover the {\em majority} of the given labelled examples. But coverage has to be weighed against the complexity of the learned hypothesis -- dramatically increasing the hypothesis complexity to cover a few more examples is in general undesirable, as these examples may well be incorrectly labeled. 

In \cite{evans2017learning}, it was claimed that ILP approaches are unable ``to handle noisy, erroneous, or ambiguous data'' and that ``If the positive or negative examples contain any mislabelled data, ILP approaches will not be able to learn the intended rule". But, approaches for performing ILP in the context of noisy examples have been presented in the literature. Examples include ~\cite{Oblak2010}, where an ILP system, called HYPER/N has been proposed to support learning from noisy data and applied to synthetic weather data for learning to predict the movement of rain from radar rain images and synoptic data. Similarly in \cite{McCreath1997} a Bayesian heuristic for finding the most probable hypotheses has been incorporated into the ILP system LIME to handle noise in the examples. All these existing systems are (i) confined to the traditional notion of ILP where knowledge is expressed as definite logic programs, and (ii) are {\em approximations} in the sense that they compute approximations of optimal solutions from noisy data. 
 
In this paper we show how a recently developed system, called ILASP3, is capable of learning complex knowledge, expressed as Answer set programs, from noisy data in an effective and scalable way. A collection of datasets, ranging from synthetically generated to real datasets, is used to evaluate the performance of the system with respect to increased percentage of noise in the labelled examples and compared it with respect to existing ILP frameworks, including in particular the $\delta$ILP recently proposed as scalable differential  learning approach for knowledge acquisition from noisy data~\cite{evans2017learning}.  Specifically, we consider two classes of syntactically generated datasets, called Hamiltonian graph and Journey preferences respectively, in order to control the percentage of noise in the data and investigate how investigate how the performance of ILASP3 varies with the amount of noise ini the examples. We show that ILASP3 approach is able in both cases to achieve a high accuracy (of well over 90\%), even with 20\% of the examples labeled incorrectly. We then evaluate ILASP on the CAVIAR dataset ~\cite{} for learning knowledge about initiating and  terminating conditions for two people meetings from data gathered from a video stream. Results show that ILASP3 reached higher precision and recall given a better F1 score than that reached by existing ILP system OLED (\cite{OLED}).  Other two real datasets are in the domain of sentence chunking~\cite{} where the task is to learn to split a sentence into short phrases, called chunks, and car preference learning. In the first case, the ability of ILASP3 to compute ``globally" optimal inductive solutions for a given learning task with noisy data allows it to reach higher accuracy than systems such as Inspire~\cite{} which learns approximations of an optimal solution, terminating also in less time than the Inspire's timeout. In the case of car preference learning, a car preference dataset~\cite{} was used and the task is to learn users' preference models in choosing cars out of a given set models with related features. Results show that ILASP3 can effectively learn such models with higher accuracy that existing ALEPH system~\cite{}. Finally, and most importantly, ILASP3 is compared to the differentiable $\delta$ILP method~\cite{}. Results show that ILASP3 achieves similar results to $\delta$ILP when the noise is in the range of 0\% to 40\%. However, at the other end of the scale (with more than 50\% noise), ILASP3 starts to learn the negation of the target hypothesis whereas $\delta$ILP incorrectly maintains less than 20\% of error in learning knowledge that not longer represented by the highly noisy data. 

The paper is organised as follows......

==> old_background.tex <==

Given any atoms $\asp{h, h_1,\ldots,h_k, b_1,\ldots,b_n,c_1,\ldots,c_m}$,
$\asp{h \codeif b_1,\ldots, b_n, \naf c_{1},\ldots, \naf c_{m}}$ is called a
\emph{normal rule} (``$\mathtt{not}$'' represents negation as failure); a rule
$\asp{\codeif b_1,\ldots, b_n,\naf c_{1},\ldots,\naf c_{m}}$ is a \emph{hard
constraint}; a \emph{choice rule} is a rule $\asp{l\{h_{1}, \ldots,
h_{k}\}u\codeif b_1,\ldots, b_n,\naf c_{1},\ldots, \naf c_{m}}$ (where
$\asp{l}$ and $\asp{u}$ are integers) and $\asp{l\{h_{1}, \ldots, h_{k}\}u}$ is
called an \emph{aggregate}. A \emph{weak constraint} is of the form $\asp{:\sim
b_1,\ldots,b_n, \naf c_1,\ldots,}$ $\asp{\naf c_m\ruleend[w@l,t_1,\ldots,
t_k]}$ where $\asp{b_1, \ldots, b_n}$, $\asp{c_1,\ldots,c_m}$ are atoms,
$\asp{w}$ and $\asp{l}$ are terms specifying the \emph{weight} and the
\emph{level}, and $\asp{t_1,\ldots,t_k}$ are terms.

The \emph{Herbrand Base} of any program $P$, denoted $HB_P$, is the set of
variable free (ground) atoms that can be formed from predicates and constants
in $P$. The subsets of $HB_P$ are called the (Herbrand) interpretations of $P$.
A ground aggregate $\asp{l\{h_{1}, \ldots, h_{k}\}u}$ is satisfied by an
interpretation $I$ iff $\asp{l}\leq| I\cap\{\asp{h_{1}, \ldots,h_{k}}\}|\leq
\asp{u}$.  The semantics of ASP programs are defined in terms of \emph{answer
sets} -- a special subset of the models of a program\footnote{For a formal
definition of answer sets of the programs considered in this paper,
see~\citep{simpleReduct}.}.
\emph{Weak constraints} do not affect what is, or is not, an answer set of a
program $P$. Instead, weak constraints create an ordering $\succ_{P}$ over
$AS(P)$ specifying which answer sets are ``preferred'' to others. Informally,
at each \emph{priority level} $\asp{l}$, the aim is to discard any answer set
which does not minimise the sum of the weights of the ground weak constraints
(with level $\asp{l}$) whose bodies are true. The higher levels are minimised
first.

All ASP programs in this paper are finite sets of normal rules, choice rules
and hard and weak constraints. The set $ord(P)$ captures the ordering of
interpretations induced by $P$. $ord(P)$ generalises the $\succ_{P}$ relation,
so it not only includes $\langle A_1, A_2, <\rangle$ if $A_1 \succ_{P} A_2$,
but also includes tuple for other binary comparison operators. More formally,
it is defined as follows: $\langle A_1, A_2, <\rangle \in ord(P)$ if $A_1
\succ_{P} A_2$; $\langle A_1, A_2, >\rangle \in ord(P)$ if $A_2 \succ_{P} A_1$;
$\langle A_1, A_2, \leq\rangle \in ord(P)$ if $A_2 \not\succ_{P} A_1$; $\langle
A_1, A_2, \geq\rangle \in ord(P)$ if $A_1 \not\succ_{P} A_2$; $\langle A_1,
A_2, =\rangle \in ord(P)$ if $A_1 \not\succ_P A_2$ and $A_2 \not\succ_{P} A_1$;
$\langle A_1, A_2, \neq\rangle \in ord(P)$ if $A_1 \succ_P A_2$ or $A_2
\succ_{P} A_1$.

%\subsection{Learning Answer Set Programs}

A \emph{partial interpretation} $e$ is a pair of sets of atoms $\langle
e^{inc}, e^{exc}\rangle$. An interpretation $I$ is said to \emph{extend} $e$
iff $e^{inc} \subseteq I$ and $e^{exc} \cap I = \emptyset$.  A
context-dependent partial interpretation (CDPI) $ex$ is a pair $\langle
ex_{pi}, ex_{ctx}\rangle$, where $ex_{pi}$ is a partial interpretation and
$ex_{ctx}$ is a program, consisting of normal rules, choice rules and hard
constraints, called the context of $ex$. A program $P$ is said to \emph{accept}
$ex$ if there is at least one answer set $A$ of $P \cup ex_{ctx}$ that extends
$ex_{pi}$ -- such an $A$ is called an accepting answer set of $P$ wrt $ex$.  A
\emph{context-dependent ordering example} (CDOE) $o$ is a tuple $\langle ex_1,
ex_2, op\rangle$, where the first two elements are CDPIs and op is a binary
comparison operator ($<$, $>$, $=$, $\leq$, $\geq$ or $\neq$).  A program $P$
is said to \emph{bravely respect} $o$ if there is a pair of accepting answer
sets, $A_1$ and $A_2$, of $P$ wrt $ex_1$ and $ex_2$, respectively, such that
$\langle A_1, A_2, op\rangle \in ord(P)$.  A program $P$ is said to
\emph{cautiously respect} $o$ if for every pair of accepting answer sets, $A_1$
and $A_2$, of $P$ (wrt $ex_1$ and $ex_2$, respectively), $\langle A_1, A_2,
op\rangle \in ord(P)$.

A learning task consists of an ASP background knowledge, CDPI and CDOE examples
and a hypothesis space, which defines the set of rules which are allowed to be
used in constructing solutions of the task. In practice, hypothesis spaces are
usually specified using mode declarations\footnote{For details of hypothesis
spaces in this paper, see
\url{https://www.doc.ic.ac.uk/~ml1909/ILASP/}.}.
%
%\begin{definition} \label{def:loas_context}
  A \emph{Context-dependent Learning
  from Ordered Answer Sets} ($ILP_{LOAS}^{context}$) task is a tuple $T=\langle
  B, S_M,\langle E^{+}, E^{-},O^{b}, O^{c}\rangle\rangle$ where $B$ is an ASP
  program called the background knowledge, $S_{M}$ is the set of rules allowed
  in the hypotheses (the hypothesis space), $E^{+}$ and $E^{-}$ are finite sets
  of CDPIs called, respectively, positive and negative examples, and $O^{b}$
  and $O^{c}$ are finite sets of CDOEs over $E^{+}$ called, respectively, brave
  and cautious context-dependent orderings. A hypothesis $H \subseteq S_M$ is
  an inductive solution of $T$ (written $H \in ILP_{LOAS}^{context}(T)$) if and
  only if:
  %\begin{enumerate}
    %\item
      (a) $\forall e^{+} \in E^{+}$, $B\cup H$ accepts $e^{+}$;
    %\item
      (b) $\forall e^{-} \in E^{-}$, $B\cup H$ does not accept $e^{-}$;
    %\item
      (c) $\forall o \in O^b$, $B\cup H$ bravely respects $o$; and,
    %\item
      (d) $\forall o \in O^c$, $B\cup H$ cautiously respects $o$.
  %\end{enumerate}
%
  The set of \emph{optimal inductive solutions} of $T$ (written
  $^*ILP_{LOAS}^{context}(T)$) is the set of inductive solutions $H\in
  ILP_{LOAS}^{context}(T)$ such that there is no other inductive solution $H'$
  such that $|H| > |H'|$.
%\end{definition}
%
We say that an example $e$ is \emph{covered} by a hypothesis $H$ if the
condition for $e$ is met by $H$; for instance, a positive example $e^+$ is
covered by $H$ if and only if $B\cup H$ accepts $e^+$.
%
ILASP (Inductive Learning of Answer Set Programs,
\citep{JELIAILASP,ILASP_system}) is a collection of algorithms for solving
$ILP_{LOAS}^{context}$ tasks. The most recent ILASP algorithm, ILASP3,
iteratively translates examples into \emph{hypothesis constraints} --
constraints on the structure of a hypothesis that are satisfied if and only if
the hypothesis covers the example.

